Aligning Agentic World Models via Knowledgeable Experience Learning

Current Large Language Models (LLMs) exhibit a critical modal disconnect: they possess vast semantic knowledge but lack the procedural grounding to respect the immutable laws of the physical world. Consequently, while these agents implicitly function as world models, their simulations often suffer from physical hallucinations-generating plans that are logically sound but physically unexecutable. Existing alignment strategies predominantly rely on resource-intensive training or fine-tuning, which attempt to compress dynamic environmental rules into static model parameters. However, such parametric encapsulation is inherently rigid, struggling to adapt to the open-ended variability of physical dynamics without continuous, costly retraining. To bridge this gap, we introduce WorldMind, a framework that autonomously constructs a symbolic World Knowledge Repository by synthesizing environmental feedback. Specifically, it unifies Process Experience to enforce physical feasibility via prediction errors and Goal Experience to guide task optimality through successful trajectories. Experiments on EB-ALFRED and EB-Habitat demonstrate that WorldMind achieves superior performance compared to baselines with remarkable cross-model and cross-environment transferability.

==> tables/main2.tex <==
% \begin{table*}[t]
% \small
% \centering


% \setlength{\tabcolsep}{4pt} % 调整列间距

% % --- 已修改：添加了竖线 (ll|cccc|cc) ---
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll|cccc|cc} 
% \toprule

% % --- 多行表头 ---
% % \multirow{2}{*}{...} 让前两列纵向跨越 2 行
% \multirow{2}{*}{\textbf{Task Group}} & \multirow{2}{*}{\textbf{Task / Metric}} & \multicolumn{4}{c|}{\textbf{Backbone}} & \multicolumn{2}{c}{\textbf{AWM}} \\ 
% \cmidrule(lr){3-6} \cmidrule(lr){7-8} % 在 "backbone/ours" 和具体模型间画线
% % 前两列留空 (因为被 multirow 占据), 然后列出具体模型名称
% & & \textbf{GPT-4o-mini} & \textbf{GPT-4o} & \textbf{Gemini 2.0 Flash} & \textbf{Qwen-VL-Plus} &\textbf{GPT-4o-mini} & \textbf{deepseek-v3.2-exp}  \\ 
% \midrule

% % --- 第1部分：Outdoor Tasks ---
% \multirow{12}{*}{\rotatebox{90}{\textbf{Outdoor Tasks}}} 
% & \textbf{Navigation} & & & & & & \\ % 子任务1
% % --- 已修改：指标改为斜体 ---
% & \quad \textit{Overall Acc} & & & & & & \\ 
% & \quad \textit{Completion Rate} & & & & & & \\ 
% & \quad \textit{Web Acc} & & & & & & \\ 
% & \quad \textit{Embodied Acc} & & & & & & \\ 

% \addlinespace[3pt] % <-- 在线上方添加 3pt 间距
% \cdashline{2-8} % 在子任务间画一条虚线分割线
% \addlinespace[3pt] % <-- 在线下方添加 3pt 间距

% & \textbf{Shopping} & & & & & & \\ % 子任务2
% % --- 已修改：指标改为斜体 ---
% & \quad \textit{Overall Acc} & & & & & & \\ 
% & \quad \textit{Completion Rate} & & & & & & \\ 
% & \quad \textit{Web Acc} & & & & & & \\ 
% & \quad \textit{Embodied Acc} & & & & & & \\ 

% \addlinespace[3pt] % <-- 在线上方添加 3pt 间距
% \cdashline{2-8} % 在子任务间画一条虚线分割线
% \addlinespace[3pt] % <-- 在线下方添加 3pt 间距

% & \textbf{Traveling} & & & & & & \\ % 子任务3
% % --- 已修改：指标改为斜体 ---
% & \quad \textit{Overall Acc} & & & & & & \\ 
% & \quad \textit{Completion Rate} & & & & & & \\ 
% & \quad \textit{Web Acc} & & & & & & \\ 
% & \quad \textit{Embodied Acc} & & & & & & \\ 

% \midrule % --- 主分割线 ---

% % --- 第2部分：Cooking Task ---
% \multirow{8}{*}{\rotatebox{90}{\textbf{Indoor Task}}} 
% & \textbf{Cooking (Vision)} & & & & & & \\ % 子类1 (来自Table 3)
% % --- 已修改：指标改为斜体 ---
% & \quad \textit{Overall Acc} & & & & & & \\ 
% & \quad \textit{Completion Rate} & & & & & & \\ 
% & \quad \textit{Web Acc} & & & & & & \\ 
% & \quad \textit{Embodied Acc} & & & & & & \\ 

% \addlinespace[3pt] % <-- 在线上方添加 3pt 间距
% \cdashline{2-8} % 在子任务间画一条虚线分割线
% \addlinespace[3pt] % <-- 在线下方添加 3pt 间距

% & \textbf{Cooking (Text)} & & & & & & \\ % 子类2 (来自Table 3)
% % --- 已修改：指标改为斜体 ---
% & \quad \textit{Overall Acc} & & 38.98 & & & 39.98 & \\ 
% & \quad \textit{Completion Rate} & & & & & & \\ 
% & \quad \textit{Web Acc} & & & & & & \\ 
% & \quad \textit{Embodied Acc} & & & & & & \\ 

% \bottomrule
% \end{tabular}
% }
% \caption{Model Performance Across Different Outdoor and Indoor Tasks} % 替换为你想要的标题
% \label{tab:merged_performance} % Label 应该放在 Caption 之后

% \end{table*}






\begin{table}[t]
\centering
\small

% 调整列间距以适应单栏宽度
\setlength{\tabcolsep}{4pt} 
\renewcommand{\arraystretch}{1.2}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc} 
\toprule

% --- 第一行表头：模型名称 ---
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c|}{\textbf{GPT-3.5-turbo}} & \multicolumn{2}{c}{\textbf{GPT-4.1-mini}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}

% --- 第二行表头：方法名称 ---
& \textbf{ReAct} & \textbf{WorldMind} & \textbf{ReAct} & \textbf{WorldMind} \\ 
\midrule

% --- 任务标识 (Indoor Cooking Text) ---
\multicolumn{5}{c}{\textbf{Indoor Task: Cooking (Text)}} \\
\midrule

% --- 数据行 (请填入具体数值) ---
\textit{Overall Acc}     & 9.82  & 20.54 & 11.61 & 24.11 \\ 
\textit{Completion Rate} & 17.02 & 39.99 & 21.88 & 41.50 \\ 
\textit{Web Acc}         & 33.93 & 45.54 & 45.54 & 80.36 \\ 
\textit{Embodied Acc}    & 29.99 & 48.70 & 32.17 & 47.27 \\ 

\bottomrule
\end{tabular}
}
\caption{Performance comparison on the Indoor Cooking (Text) task. We evaluate both ReAct baseline and our WorldMind using GPT-3.5-turbo and GPT-4.1-mini backbones.} 
\label{tab:indoor_comparison}
\end{table}


